String Diagrammatic Electrical Circuit Theory

We develop a comprehensive string diagrammatic treatment of electrical circuits. Building on previous, limited case studies, we introduce controlled sources and meters as elements, and the impedance calculus, a powerful toolbox for diagrammatic reasoning on circuit diagrams. We demonstrate the power of our approach by giving idiomatic proofs of several textbook results, including the superposition theorem and Thevenin's theorem.

==> eptcsdata.tex <==
\providecommand{\firstpage}{178}
\providecommand{\publicationstatus}{K. Kishida (Ed.): Fourth International Conference\\
on Applied Category Theory (ACT 2021).\\
EPTCS 372, 2022, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.372.13}{10.4204/EPTCS.372.13}}
\pdfoutput=1

